The He star donor channel towards the black widow PSR J1953+1844

Black widows (BWs) are a type of eclipsing millisecond pulsars (MSPs) with low companion masses ($\lesssim0.05\,\rm M_\odot$) and tight orbits ($<1\,$d). PSR J1953+1844 is a BW with the shortest orbital period ($\sim53$ minutes) ever discovered, which was recently detected by Five-hundred-meter Aperture Spherical radio Telescope. Its companion mass is $\sim0.01\,\rm M_\odot$ according to its mass function, indicating that the companion may be a hydrogen-deficient star. However, the origin of PSR J1953+1844 is highly unclear. In this paper, we explored the origin of PSR J1953+1844 through the neutron star+He star channel, in which the system can experience ultracompact X-ray binary phase. We found that the He star donor channel can reproduce the characteristics of PSR J1953+1844, indicating that this work provides an alternative formation channel for this source. Meanwhile, the minimum orbital period of BWs formed by this channel is $\sim28$ minutes, corresponding to the companion mass of $0.058\,\rm M_\odot$. In addition, we note that even though PSR J1953+1844 has a short orbital period, it cannot be detected by the gravitational wave (GW) observatories like Laser Interferometer Space Antenna, TaiJi and TianQin. However, we still expect that the BWs with extremely tight orbit produced by this channel are the potential sources of future space-based GW observatories. Moreover, our simulations show that PSR J1953+1844 may eventually evolve into an isolated MSP.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

